TS-Detector : Detecting Feature Toggle Usage Patterns

Feature toggles enable developers to control feature states, allowing the features to be released to a limited group of users while preserving overall software functionality. The absence of comprehensive best practices for feature toggle usage often results in improper implementation, causing code quality issues. Although certain feature toggle usage patterns are prone to toggle smells, there is no tool as of today for software engineers to detect toggle usage patterns from the source code. This paper presents a tool TS-Detector to detect five different toggle usage patterns across ten open-source software projects in six different programming languages. We conducted a manual evaluation and results show that the true positive rates of detecting Spread, Nested, and Dead toggles are 80%, 86.4%, and 66.6% respectively, and the true negative rate of Mixed and Enum usages was 100%. The tool can be downloaded from its GitHub repository and can be used following the instructions provided there.

==> 05_analysis.tex <==
\section{Analysis}
To analyze the influence of toggle usage patterns on code complexity we collected two datasets. 
The first dataset was collected using Understand API~\cite{understandapi}.
The second dataset is collected by running our ts-detector tool on Chromium and Dawn source code where we collected toggle usages counts per file. 

\subsection{Complexity Metrics}
The powerful python-based API provided by Scitools for the popular static analysis tool \textit{Understand} allowed us to conveniently extract the code quality metrics---average Cyclomatic Complexity per file (CC), average lines of code in methods per file (AvgLOC),
number of inactive lines per file (ILOC),
Executable LOC per file (ExLOC),
and Maximum Nesting level of control constructs per file (MNesting). 
The code metrics are also collected at the file level including both class files, and non-class files. 

Table~\ref{tab:codemetrics} presents code quality metrics obtained from Chromium and Dawn projects.
In the median case, each file in Chromium has an average cyclomatic complexity of 1 with a maximum of 70; on the other hand, Dawn has a similar median complexity with a maximum of 205.
Although the Chromium project is larger than Dawn in terms of code size (25GB and 0.5GB of disk space, respectively), each file in Chromium has 8 AvgLOC, while Dawn has 10 in the median case. 
%\todo{this looks quite fishy! 8 lines of code per file (median)!}
Clearly, Dawn's files are much larger since it has 1.17 times more Executable LOC (ExLOC) than Chromium.
However, the median MNesting (maximum nesting) in all Dawn files is 1, while Chromium has 2. 
%\todo{are we sure median is not minimum! These numbers seem quite low to me.}


\begin{table}[htbp]
\caption{Chromium and Dawn Code-Metrics}
\begin{center}
\label{tab:codemetrics}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
{} & CC & AvgLOC & ILOC & ExLOC & MNesting \\
\hline
\multicolumn{6}{|c|}{\textbf{Chromium}} \\
\hline
Median & 1 & 8 & 0 & 12 & 1 \\
\hline
Max & 70 & 682 & 3563 & 1703 & 10 \\
\hline
\multicolumn{6}{|c|}{\textbf{Dawn}} \\
\hline
Median & 1 & 10 & 0 & 8 & 0 \\
\hline
Max & 205 & 4572 & 577 & 2006 & 8 \\
\hline
\end{tabular}
\end{center}
\end{table}

Table~\ref{tab:codemetrics2} presents code quality metrics obtained from Sentry in Python, React in JavaScript, and OpenSearch in Java. Unfortunately, Scitools is not currently supporting Go, so we can not get an analysis on Cadence to compare. The ILOC is also not available to projects that are not in C/C++, therefore we will only compare the rest 4 fields between these projects in this table. These three projects are in similar sizes ranging from 500MB to 750MB in terms of disk space.
In terms of Average Lines of Code (AvgLOC), React displays the most disparate values, with a median of 1 but a maximum of 7606, surpassing the respective maximums of 252 for Sentry and 578 for OpenSearch. Concerning Executable Lines of Code (ExLOC), OpenSearch boasts the highest median value of 22, compared to 7 for Sentry and 4 for React. However, both CC and MNesting exhibit relatively similar maximum and median values across the three projects.

\begin{table}[htbp]
\caption{Sentry, React and OpenSearch Code-Metrics}
\begin{center}
\label{tab:codemetrics2}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
{} & CC & AvgLOC & ExLOC & MNesting \\
\hline
\multicolumn{5}{|c|}{\textbf{Sentry}} \\
\hline
Median & 1 & 8 & 7 & 1 \\
\hline
Max & 19 & 252 & 2481 & 10 \\
\hline

\multicolumn{5}{|c|}{\textbf{React}} \\
\hline
Median & 1 & 1 & 4 & 0 \\
\hline
Max & 30 & 7606 & 2273 & 8 \\
\hline

\multicolumn{5}{|c|}{\textbf{OpenSearch}} \\
\hline
Median & 1 & 7 & 22 & 1 \\
\hline
Max & 31 & 578 & 3894 & 10 \\
\hline
\end{tabular}
\end{center}
\end{table}


Many code metrics have been studied as complexity metrics in the literature~\cite{magel1982applying,kafura1987use,debbarma2013review,yi2020complexity} while cyclomatic complexity has always been popular among both researchers and practitioners.
However, we have included AvgLOC metrics as well along with maximum nesting (MNesting) metrics since toggles may cause nesting, create additional lines of code, leave dead code, and may contribute to the increase of cyclomatic complexity. 

\subsection{Quantify Toggle Usages}
To quantify the toggle usages, we ran our tool \textit{ts-detector} on the source code of all six projects mentioned above. 
Following is a snippet of the JSON output of \textit{ts-detector} resulting from the command to analyze Cadence for spread toggles.
% \begin{center}
%     ``\textit{python3 tsd.py C++ ~/Downloads/chromium/ switches.cc spread}''
% \end{center}

\begin{lstlisting}[language=Go, caption={ts-detector output for nested toggles in Cadence}]
  {
    "Nested_Toggles": {
        ...
        "archival.go": [
          "common.ArchivalEnabled",
          "a.History.EnableRead",
          "EnableRead",
          "a.Visibility.EnableRead"
        ],
        "authorization.go": [
          "a.OAuthAuthorizer.Enable",
          "a.NoopAuthorizer.Enable"
        ],
        "attrValidator.go": [
          "types.ArchivalStatusEnabled",
          "d.clusterMetadata.GetEnabledClusterInfo"
        ],
        "versionChecker.go": [
          "featureFlags.WorkflowExecutionAlreadyCompletedErrorEnabled",
          "flags.WorkflowExecutionAlreadyCompletedErrorEnabled",
          "*featureFlags.WorkflowExecutionAlreadyCompletedErrorEnabled"
        ]
  },
  "total_count_path": 22,
  "total_count_toggles": 38
}
\end{lstlisting}

The toggle variable is one of the two keys of the output JSON.
Each toggle key contains a dictionary of file paths where the usage instances of that key toggle variable been has found. 
The total count path and total count toggles are also collected as separate keys for convenience. The total count path represents how many files are there using nested toggles and the total count toggles represents the amount of toggles used in a nested pattern.

We collected these JSON outputs and stored in data tables for each four toggle usage patterns.
Each table contains the file name where the toggle usage was found, and the count of how many usage instances were found.
We then map the two datasets (one using \textit{Understand}, and another using our \textit{ts-detector}) and merge into one final dataset for our analysis.
% The following text is, in my opinion, not required. It might confuse people.
% Table~\ref{tab:finaldataset} shows a snippet of this data table where all code quality metrics and the toggle usages counts are in columns for each file.

% \begin{table*}[htbp]
% \caption{Final dataset : Toggle usages and Code metrics}
% \begin{center}
% \label{tab:finaldataset}
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
% \hline
% \textbf{File} & \textbf{CC} & \textbf{AvgLOC} & \textbf{ILOC} & \textbf{ExLOC} & \textbf{MNesting} & \textbf{Dead} & \textbf{Spread} & \textbf{Nested} & \textbf{Mixed} \\
% \hline
% accelerator\_table.cc & 3 & 12 & 78 & 18 & 2 & 0 & 4 & 0 & 4 \\
% \hline
% about\_ui.cc & 2 & 9 & 451 & 43 & 2 & 0 & 2 & 4 & 0 \\
% \hline
% appmodel\_utils.cc & 2 & 10 & 0 & 12 & 1 & 0 & 4 & 1 & 2 \\
% \hline
% app\_service\_metrics.cc & 6 & 35 & 34 & 83 & 1 & 1 & 4 & 2 & 3 \\
% \hline
% \end{tabular}
% \end{center}
% \end{table*}

